Improving Semantic Segmentation in Transformers using Hierarchical Inter-Level Attention

Existing transformer-based image backbones typically propagate feature information in one direction from lower to higher-levels. This may not be ideal since the localization ability to delineate accurate object boundaries, is most prominent in the lower, high-resolution feature maps, while the semantics that can disambiguate image signals belonging to one object vs. another, typically emerges in a higher level of processing. We present Hierarchical Inter-Level Attention (HILA), an attention-based method that captures Bottom-Up and Top-Down Updates between features of different levels. HILA extends hierarchical vision transformer architectures by adding local connections between features of higher and lower levels to the backbone encoder. In each iteration, we construct a hierarchy by having higher-level features compete for assignments to update lower-level features belonging to them, iteratively resolving object-part relationships. These improved lower-level features are then used to re-update the higher-level features. HILA can be integrated into the majority of hierarchical architectures without requiring any changes to the base model. We add HILA into SegFormer and the Swin Transformer and show notable improvements in accuracy in semantic segmentation with fewer parameters and FLOPS. Project website and code: https://www.cs.toronto.edu/~garyleung/hila/

==> figures/ablation_tables/ablation_effect_of_updates_full3.tex <==
\begin{table}[]
\begin{center}
\caption{\textbf{Performance vs. Stage of Update}}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{|c|cc|c|c|}
\hline
\textbf{Bottom-Up}     & \multicolumn{2}{c|}{\textbf{Top-Down}}                 & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}mIOU \\ (SS)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}F-Score\\ 3px (SS)\end{tabular}} \\ \cline{1-3}
Inter-Stage Attention  & \multicolumn{1}{c|}{Inter-Stage Attention} & Transformer Layer     &      &                       \\ \hline
\multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{}                      & \multicolumn{1}{l|}{} & 78.5 & 71.4                  \\
\cmark              & \multicolumn{1}{l|}{}                      & \multicolumn{1}{l|}{} & 79.9 & 73.0                  \\
\multicolumn{1}{|l|}{} & \multicolumn{1}{c|}{\cmark} & \multicolumn{1}{l|}{} & 75.7                                & \multicolumn{1}{l|}{}             \\
\multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{}                      & \cmark             & 75.2 & \multicolumn{1}{l|}{} \\
\cmark              & \multicolumn{1}{l|}{}                      & \cmark             & 80.1 & \multicolumn{1}{l|}{} \\
\multicolumn{1}{|l|}{} & \multicolumn{1}{c|}{\cmark}             & \cmark             & 76.6 & 69.6                  \\
\cmark              & \multicolumn{1}{c|}{\cmark}             & \cmark             & 80.8 & 74.5                  \\ \hline
\end{tabular}
\end{adjustbox}
\label{table:fullyconnectedcomplexity}
\end{center}
\end{table}

==> figures/ablation_tables/ablation_first_td_skip4.tex <==
\begin{table}[]
\begin{center}
\caption{\textbf{Performance vs. Local Patch Size}}
\begin{adjustbox}{width=0.5\textwidth}
\begin{tabular}{|c|c|c|c|c|}
\hline
\begin{tabular}[c]{@{}c@{}}Skip First \\ Top-Down \\ Update\end{tabular} & Params (M) & FLOPS ↓ & \begin{tabular}[c]{@{}c@{}}mIOU \\ (SS)\end{tabular} & \begin{tabular}[c]{@{}c@{}}F-Score\\ 3px (SS)\end{tabular} \\ \hline
\xmark     &            &         &           &         \\
\cmark           &            &         & 80.8      & 74.5    \\ \hline
\end{tabular}
\end{adjustbox}
\label{table:fullyconnectedcomplexity}
\end{center}
\end{table}

==> figures/ablation_tables/ablation_fpn7.tex <==
\begin{table}[]
\begin{center}
\caption{\textbf{Performance vs. Momentum Weights}}
\begin{adjustbox}{width=0.5\textwidth}
\begin{tabular}{|c|c|c|}
\hline
Model           & mIOU (SS)                 & F1 (SS)                   \\ \hline
Segformer       & \multicolumn{1}{c|}{78.5} & \multicolumn{1}{c|}{71.4} \\
Ours            & \multicolumn{1}{c|}{80.8} & \multicolumn{1}{c|}{74.5} \\ \hline
Segformer + FPN &                           &                           \\
Ours + FPN      &                           &                           \\ \hline
\end{tabular}
\end{adjustbox}
\label{table:fullyconnectedcomplexity}
\end{center}
\end{table}

==> figures/tables/ablation_momentum.tex <==
\begin{table}[]
\begin{center}
\caption{Ablation: Effect of momentum in our update \gary{Perhaps an Appendix table?}}
\begin{adjustbox}{width=0.5\textwidth}
\label{table:ablationmomentum}
\begin{tabular}{|l|l|l|}
\hline
Momentum   & mIOU (SS) & F1 (SS) \\ \hline
(1.0, 1.0) & MISSING   &         \\ \hline
(0.2, 0.8) & MISSING   &         \\ \hline
(0.5, 0.5) & MISSING   &         \\ \hline
(0.8, 0.2) & MISSING   &         \\ \hline
\end{tabular}
\end{adjustbox}
\end{center}
\end{table}

==> figures/tables/ablation_patchsize.tex <==
\begin{table}[]
\begin{center}
\caption{Ablation: Effect of patch size in our update \gary{Perhaps an Appendix table?}}
\begin{adjustbox}{width=0.5\textwidth}
\label{table:ablationpatchsize}
\begin{tabular}{|r|l|l|l|l|}
\hline
\multicolumn{1}{|l|}{P} & Params (M) & FLOPS ↓ & mIOU (SS) & F1 (SS) \\ \hline
2                       &     21.6       &    417.5     & 80.7   &  74.7       \\ \hline
4                       &     21.6       &    417.8     & 80.8   &  74.5       \\ \hline
6                       &     21.6       &    418.3     & 80.8   &  74.5       \\ \hline
\end{tabular}
\end{adjustbox}
\end{center}
\end{table}

==> figures/tables/ablation_stride.tex <==
\begin{table}[]
\begin{center}
\caption{Ablation: Effect of update stride of our method \gary{Perhaps an Appendix table?}}
\begin{adjustbox}{width=0.5\textwidth}
\label{table:ablationstride}
\begin{tabular}{|r|l|l|l|l|}
\hline
\multicolumn{1}{|l|}{Stride Size} & Params (M) & FLOPS ↓ & mIOU (SS) & F1 (SS) \\ \hline
1                                 &            &         & MISSING   &         \\ \hline
2                                 &            &         & MISSING   &         \\ \hline
3                                 &            &         & MISSING   &         \\ \hline
\end{tabular}
\end{adjustbox}
\end{center}
\end{table}

==> figures/tables/cityscapesc.tex <==
\begin{table}[]
\begin{center}
\caption{\textbf{Robustness of Our Method in Cityscapes-C.} We report mIOU numbers of baselines from \cite{} and \cite{}.}
\begin{adjustbox}{width=\textwidth}
\label{table:cityscapesc}
\begin{tabular}{|c|c|c|cccc|cccc|cccc|cccc|}
\hline
\multirow{2}{*}{\textbf{Eval}} &
  \multirow{2}{*}{\textbf{Method}} &
  \multirow{2}{*}{\textbf{Clean}} &
  \multicolumn{4}{c|}{\textbf{Blur}} &
  \multicolumn{4}{c|}{\textbf{Noise}} &
  \multicolumn{4}{c|}{\textbf{Digital}} &
  \multicolumn{4}{c|}{\textbf{Weather}} \\ \cline{4-19} 
 &               &      & Motion & Defoc & Glass & Gauss & Gauss & Impul & Shot & Speck & Bright & Contr & Satur & JPEG & Snow & Spatt & Fog  & Frost \\ \hline
\multirow{12}{*}{\begin{tabular}[c]{@{}c@{}}mIOU \\ (SS)\end{tabular}} &
  DLv3+ (MBv2) &
  72 &
  53.5 &
  49 &
  45.3 &
  49.1 &
  6.4 &
  7 &
  6.6 &
  16.6 &
  51.7 &
  46.7 &
  32.4 &
  27.2 &
  13.7 &
  38.9 &
  47.4 &
  17.3 \\
 & DLv3+ (R101)  & 77.1 & 59.1   & 56.3  & 47.7  & 57.3  & 13.2  & 13.9  & 16.3 & 36.9  & 59.2   & 54.5  & 41.5  & 37.4 & 11.9 & 47.8  & 55.1 & 22.7  \\
 & DLv3+ (X71)   & 78.6 & 64.1   & 60.9  & 52    & 60.4  & 14.9  & 10.8  & 19.4 & 41.2  & 68     & 58.7  & 47.1  & 40.2 & 18.8 & 50.4  & 64.1 & 20.2  \\ \cline{2-19} 
 & ICNet         & 65.9 & 45.8   & 44.6  & 47.4  & 44.7  & 8.4   & 8.4   & 10.6 & 27.9  & 41     & 33.1  & 27.5  & 34   & 6.3  & 30.5  & 27.3 & 11    \\
 & FCN8s         & 66.7 & 42.7   & 31.1  & 37    & 34.1  & 6.7   & 5.7   & 7.8  & 24.9  & 53.3   & 39    & 36    & 21.2 & 11.3 & 31.6  & 37.6 & 19.7  \\
 & DilatedNet    & 68.6 & 44.4   & 36.3  & 32.5  & 38.4  & 15.6  & 14    & 18.4 & 32.7  & 52.7   & 32.6  & 38.1  & 29.1 & 12.5 & 32.3  & 34.7 & 19.2  \\
 & ResNet-38     & 77.5 & 54.6   & 45.1  & 43.3  & 47.2  & 13.7  & 16    & 18.2 & 38.3  & 60     & 50.6  & 46.9  & 14.7 & 13.5 & 45.9  & 52.9 & 22.2  \\
 & PSPNet        & 78.8 & 59.8   & 53.2  & 44.4  & 53.9  & 11    & 15.4  & 15.4 & 34.2  & 60.4   & 51.8  & 30.6  & 21.4 & 8.4  & 42.7  & 34.4 & 16.2  \\
 & GSCNN         & 80.9 & 58.9   & 58.4  & 41.9  & 60.1  & 5.5   & 2.6   & 6.8  & 24.7  & 75.9   & 61.9  & 70.7  & 12   & 12.4 & 47.3  & 67.9 & 32.6  \\ \cline{2-19} 
 & SegFormer-B5  & 82.4 & 69.1   & 68.6  & 64.1  & 69.8  & 57.8  & 63.4  & 52.3 & 72.8  & 81     & 77.7  & 80.1  & 58.8 & 40.7 & 68.4  & 78.5 & 49.9  \\ \cline{2-19} 
 & SegFormer B1  & 78.5 &        &       &       &       &       &       &      &       &        &       &       &      &      &       &      &       \\
 & + \methodthree & 80.8 &        &       &       &       &       &       &      &       &        &       &       &      &      &       &      &       \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}F-Score \\ 3px (SS)\end{tabular}} &
  SegFormer-B5 &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   \\ \cline{2-19} 
 & SegFormer B1  & 71.4 &        &       &       &       &       &       &      &       &        &       &       &      &      &       &      &       \\
 & + \methodthree & 74.5 &        &       &       &       &       &       &      &       &        &       &       &      &      &       &      &       \\ \hline
\end{tabular}
\end{adjustbox}
\end{center}
\end{table}

==> figures/tables/nonrealtime.tex <==
\begin{table}[]
\begin{center}
\caption{\textbf{Comparison to state of the art methods on ADE20K and Cityscapes.} \JG{What's the difference comparing with table 2?} \gary{this is eval comparing against state-of-the-art. I'm not sure how well executed this table will be because we are missing high-end model size - so results will be reduced to match ~B2 or B1 size}}
\begin{adjustbox}{width=\textwidth}
\label{table:comparisonresults}
\begin{tabular}{|c|c|c|ccc|ccc|}
\hline
 &
   &
   &
  \multicolumn{3}{c|}{\textbf{ADE20K}} &
  \multicolumn{3}{c|}{\textbf{Cityscapes}} \\ \cline{4-9} 
\multirow{-2}{*}{\textbf{Method}} &
  \multirow{-2}{*}{\textbf{Encoder}} &
  \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Params\\ (M)\end{tabular}}} &
  \multicolumn{1}{c|}{FLOPS} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}mIOU \\ (SS)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}F-Score \\ 3px (SS)\end{tabular} &
  \multicolumn{1}{c|}{FLOPS} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}mIOU \\ (SS)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}F-Score \\ 3px (SS)\end{tabular} \\ \hline
FCN &
  ResNet-101 &
   &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
   &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
   \\ \hline
DeepLabV3+ &
  ResNet-101 &
   &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
   &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
   \\ \hline
GSCNN &
  ResNet-101 &
   &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
   &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
   \\ \hline
...etc. &
   &
   &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
   &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
   \\ \hline
SegFormer &
  {\color[HTML]{333333} MiT-B2} &
  {\color[HTML]{333333} } &
  \multicolumn{1}{c|}{{\color[HTML]{333333} }} &
  \multicolumn{1}{c|}{} &
   &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
   \\ \hline
 &
  (w/ Our Method) &
   &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
   &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
   \\ \hline
\end{tabular}
\end{adjustbox}
\end{center}
\end{table}

==> figures/tables/perclasscomparison.tex <==
\begin{table}[]
\begin{center}
\caption{\textbf{mIOU/F-score class by class comparison.} We show the improvements from adding \method{} S(3) and S(2,3,4) to the Segformer B1 baseline model. We also compare Segformer B2 to our SegFormer B1 + \method{} model, which achieves better results with 21\% less params and 50\% less flops. }
\begin{adjustbox}{width=\textwidth}
\label{table:f1comparison}
\begin{tabular}{|c|c|ccccccc|cccccc|cccccc|c|}
\hline
 &
   &
  \multicolumn{7}{c|}{\textbf{Background}} &
  \multicolumn{6}{c|}{\textbf{Vehicles}} &
  \multicolumn{6}{c|}{\textbf{Thin/Complex}} &
   \\ \cline{3-21}
\multirow{-2}{*}{\textbf{Eval}} &
  \multirow{-2}{*}{\textbf{Method}} &
  \multicolumn{1}{c|}{road} &
  \multicolumn{1}{c|}{s.walk} &
  \multicolumn{1}{c|}{build.} &
  \multicolumn{1}{c|}{wall} &
  \multicolumn{1}{c|}{veg} &
  \multicolumn{1}{c|}{terrain} &
  sky &
  \multicolumn{1}{c|}{car} &
  \multicolumn{1}{c|}{truck} &
  \multicolumn{1}{c|}{bus} &
  \multicolumn{1}{c|}{train} &
  \multicolumn{1}{c|}{motor} &
  bike &
  \multicolumn{1}{c|}{fence} &
  \multicolumn{1}{c|}{pole} &
  \multicolumn{1}{c|}{t-light} &
  \multicolumn{1}{c|}{t-sign} &
  \multicolumn{1}{c|}{person} &
  rider &
  \multirow{-2}{*}{\textbf{Mean}} \\ \hline
 &
  SegFormer B1 &
  \multicolumn{1}{c|}{83.4} &
  \multicolumn{1}{c|}{64.7} &
  \multicolumn{1}{c|}{71.2} &
  \multicolumn{1}{c|}{53.6} &
  \multicolumn{1}{c|}{73.3} &
  \multicolumn{1}{c|}{54.8} &
  \textbf{82.4} &
  \multicolumn{1}{c|}{78.6} &
  \multicolumn{1}{c|}{82.2} &
  \multicolumn{1}{c|}{87.8} &
  \multicolumn{1}{c|}{94.1} &
  \multicolumn{1}{c|}{80.4} &
  62.2 &
  \multicolumn{1}{c|}{50.4} &
  \multicolumn{1}{c|}{71.4} &
  \multicolumn{1}{c|}{67.2} &
  \multicolumn{1}{c|}{70.6} &
  \multicolumn{1}{c|}{60.8} &
  67.7 &
  71.4 \\ \cline{2-22} 
 &
   &
  \multicolumn{1}{c|}{\textbf{84.3}} &
  \multicolumn{1}{c|}{\textbf{66.2}} &
  \multicolumn{1}{c|}{\textbf{72.9}} &
  \multicolumn{1}{c|}{\textbf{55.3}} &
  \multicolumn{1}{c|}{\textbf{74.0}} &
  \multicolumn{1}{c|}{\textbf{55.5}} &
  \textbf{83.1} &
  \multicolumn{1}{c|}{\textbf{81.2}} &
  \multicolumn{1}{c|}{\textbf{82.7}} &
  \multicolumn{1}{c|}{\textbf{88.3}} &
  \multicolumn{1}{c|}{\textbf{95.8}} &
  \multicolumn{1}{c|}{\textbf{78.6}} &
  \textbf{64.8} &
  \multicolumn{1}{c|}{\textbf{54.6}} &
  \multicolumn{1}{c|}{\textbf{74.8}} &
  \multicolumn{1}{c|}{\textbf{73.5}} &
  \multicolumn{1}{c|}{\textbf{73.8}} &
  \multicolumn{1}{c|}{\textbf{65.5}} &
  \textbf{69.3} &
  \textbf{73.4} \\
 &
  \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}SegFormer B1 \\ + \methodone{}\end{tabular}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+0.9}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+1.5}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+1.7}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+1.7}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+0.7}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+0.7}}} &
  {\color[HTML]{036400} \textbf{+0.7}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+2.6}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+0.5}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+0.5}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+1.7}}} &
  \multicolumn{1}{c|}{{\color[HTML]{9A0000} \textbf{-1.8}}} &
  {\color[HTML]{036400} \textbf{+2.6}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+4.2}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+3.4}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+6.3}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+3.2}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+4.7}}} &
  {\color[HTML]{036400} \textbf{+1.6}} &
  {\color[HTML]{036400} \textbf{+2.0}} \\ \cline{2-22} 
 &
   &
  \multicolumn{1}{c|}{\textbf{84.4}} &
  \multicolumn{1}{c|}{\textbf{68.3}} &
  \multicolumn{1}{c|}{\textbf{74.3}} &
  \multicolumn{1}{c|}{\textbf{61.9}} &
  \multicolumn{1}{c|}{\textbf{74.6}} &
  \multicolumn{1}{c|}{\textbf{57.7}} &
  82.5 &
  \multicolumn{1}{c|}{\textbf{82.4}} &
  \multicolumn{1}{c|}{\textbf{83.1}} &
  \multicolumn{1}{c|}{\textbf{91.5}} &
  \multicolumn{1}{c|}{\textbf{97.5}} &
  \multicolumn{1}{c|}{\textbf{83.7}} &
  \textbf{67.6} &
  \multicolumn{1}{c|}{\textbf{56.9}} &
  \multicolumn{1}{c|}{\textbf{75.8}} &
  \multicolumn{1}{c|}{\textbf{78.5}} &
  \multicolumn{1}{c|}{\textbf{73.9}} &
  \multicolumn{1}{c|}{\textbf{66.0}} &
  \textbf{71.9} &
  \textbf{74.8} \\
\multirow{-5}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}F-Score \\ 3px (SS)\end{tabular}}} &
  \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}SegFormer B1 \\ + \methodthree{}\end{tabular}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+1.0}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+3.6}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+3.1}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+8.3}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+1.3}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+2.9}}} &
  {\color[HTML]{036400} \textbf{+0.1}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+3.8}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+0.9}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+3.7}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+3.4}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+3.3}}} &
  {\color[HTML]{036400} \textbf{+5.4}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+6.5}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+4.4}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+11.3}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+3.3}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+5.2}}} &
  {\color[HTML]{036400} \textbf{+4.2}} &
  {\color[HTML]{036400} \textbf{+3.4}} \\ \hline
 &
  SegFormer B1 &
  \multicolumn{1}{c|}{98.3} &
  \multicolumn{1}{c|}{85.7} &
  \multicolumn{1}{c|}{92.6} &
  \multicolumn{1}{c|}{58.7} &
  \multicolumn{1}{c|}{92.8} &
  \multicolumn{1}{c|}{65.1} &
  \textbf{95.3} &
  \multicolumn{1}{c|}{95.2} &
  \multicolumn{1}{c|}{82.7} &
  \multicolumn{1}{c|}{87.3} &
  \multicolumn{1}{c|}{74.2} &
  \multicolumn{1}{c|}{68.1} &
  78.0 &
  \multicolumn{1}{c|}{58.5} &
  \multicolumn{1}{c|}{65.4} &
  \multicolumn{1}{c|}{71.8} &
  \multicolumn{1}{c|}{79.9} &
  \multicolumn{1}{c|}{82.0} &
  60.1 &
  \textbf{78.5} \\ \cline{2-22} 
 &
   &
  \multicolumn{1}{c|}{\textbf{98.4}} &
  \multicolumn{1}{c|}{86.5} &
  \multicolumn{1}{c|}{93.1} &
  \multicolumn{1}{c|}{63.7} &
  \multicolumn{1}{c|}{92.9} &
  \multicolumn{1}{c|}{\textbf{65.6}} &
  \textbf{95.3} &
  \multicolumn{1}{c|}{95.4} &
  \multicolumn{1}{c|}{83.6} &
  \multicolumn{1}{c|}{89.3} &
  \multicolumn{1}{c|}{\textbf{81.2}} &
  \multicolumn{1}{c|}{68.9} &
  78.9 &
  \multicolumn{1}{c|}{60.8} &
  \multicolumn{1}{c|}{67.4} &
  \multicolumn{1}{c|}{73.3} &
  \multicolumn{1}{c|}{81.3} &
  \multicolumn{1}{c|}{83.6} &
  63.9 &
  80.2 \\
 &
  \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}SegFormer B1 \\ + \methodone{}\end{tabular}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+0.1}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+0.8}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+0.5}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+5.0}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+0.1}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+0.5}}} &
  {\color[HTML]{036400} \textbf{+0.0}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+0.2}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+0.9}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+2.0}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+7.0}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+0.8}}} &
  {\color[HTML]{036400} \textbf{+0.9}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+2.3}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+2.0}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+1.5}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+1.4}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+1.6}}} &
  {\color[HTML]{036400} \textbf{+3.8}} &
  {\color[HTML]{036400} \textbf{+1.7}} \\ \cline{2-22} 
 &
   &
  \multicolumn{1}{c|}{98.3} &
  \multicolumn{1}{c|}{\textbf{86.6}} &
  \multicolumn{1}{c|}{\textbf{93.4}} &
  \multicolumn{1}{c|}{\textbf{67.7}} &
  \multicolumn{1}{c|}{\textbf{93.1}} &
  \multicolumn{1}{c|}{\textbf{64.9}} &
  \textbf{95.2} &
  \multicolumn{1}{c|}{\textbf{95.6}} &
  \multicolumn{1}{c|}{\textbf{86.2}} &
  \multicolumn{1}{c|}{\textbf{89.4}} &
  \multicolumn{1}{c|}{\textbf{79.7}} &
  \multicolumn{1}{c|}{\textbf{69.5}} &
  \textbf{79.1} &
  \multicolumn{1}{c|}{\textbf{63.5}} &
  \multicolumn{1}{c|}{\textbf{68.8}} &
  \multicolumn{1}{c|}{\textbf{74.4}} &
  \multicolumn{1}{c|}{\textbf{81.4}} &
  \multicolumn{1}{c|}{\textbf{84.2}} &
  \textbf{66.5} &
  \textbf{80.9} \\
\multirow{-5}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}mIOU \\ (MS)\end{tabular}}} &
  \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}SegFormer B1 \\ + \methodthree{}\end{tabular}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+0.0}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+0.9}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+0.8}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+9.0}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+0.3}}} &
  \multicolumn{1}{c|}{{\color[HTML]{9A0000} \textbf{-0.2}}} &
  {\color[HTML]{036400} \textbf{-+0.1}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+0.4}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+3.5}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+2.1}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+5.5}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+1.4}}} &
  {\color[HTML]{036400} \textbf{+1.1}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+5.0}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+3.4}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+2.6}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+1.5}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+2.2}}} &
  {\color[HTML]{036400} \textbf{+6.4}} &
  {\color[HTML]{036400} \textbf{+2.4}} \\ \hline
 &
  SegFormer B2 &
  \multicolumn{1}{c|}{\textbf{84.6}} &
  \multicolumn{1}{c|}{67.2} &
  \multicolumn{1}{c|}{74.2} &
  \multicolumn{1}{c|}{55.2} &
  \multicolumn{1}{c|}{\textbf{75.2}} &
  \multicolumn{1}{c|}{57.4} &
  \textbf{83.3} &
  \multicolumn{1}{c|}{82.1} &
  \multicolumn{1}{c|}{82.4} &
  \multicolumn{1}{c|}{90.1} &
  \multicolumn{1}{c|}{95.9} &
  \multicolumn{1}{c|}{77.8} &
  66.4 &
  \multicolumn{1}{c|}{54.5} &
  \multicolumn{1}{c|}{\textbf{76.8}} &
  \multicolumn{1}{c|}{74.9} &
  \multicolumn{1}{c|}{\textbf{74.7}} &
  \multicolumn{1}{c|}{\textbf{67.3}} &
  70.5 &
  74.2 \\ \cline{2-22} 
 &
   &
  \multicolumn{1}{c|}{84.4} &
  \multicolumn{1}{c|}{\textbf{68.3}} &
  \multicolumn{1}{c|}{\textbf{74.3}} &
  \multicolumn{1}{c|}{\textbf{61.9}} &
  \multicolumn{1}{c|}{74.6} &
  \multicolumn{1}{c|}{\textbf{57.7}} &
  82.5 &
  \multicolumn{1}{c|}{\textbf{82.4}} &
  \multicolumn{1}{c|}{\textbf{83.1}} &
  \multicolumn{1}{c|}{\textbf{91.5}} &
  \multicolumn{1}{c|}{\textbf{97.5}} &
  \multicolumn{1}{c|}{\textbf{83.7}} &
  \textbf{67.6} &
  \multicolumn{1}{c|}{\textbf{56.9}} &
  \multicolumn{1}{c|}{75.8} &
  \multicolumn{1}{c|}{\textbf{78.5}} &
  \multicolumn{1}{c|}{73.9} &
  \multicolumn{1}{c|}{66.0} &
  \textbf{71.9} &
  \textbf{74.8} \\
\multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}F-Score \\ 3px (SS)\end{tabular}}} &
  \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}SegFormer B1 \\ + \methodthree{}\end{tabular}} &
  \multicolumn{1}{c|}{{\color[HTML]{9A0000} \textbf{-0.2}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+1.1}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+0.1}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+6.7}}} &
  \multicolumn{1}{c|}{{\color[HTML]{9A0000} \textbf{-0.6}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+0.3}}} &
  {\color[HTML]{9A0000} \textbf{-0.8}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+0.3}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+0.7}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+1.4}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+1.6}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+5.9}}} &
  {\color[HTML]{036400} \textbf{+1.2}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+2.4}}} &
  \multicolumn{1}{c|}{{\color[HTML]{9A0000} \textbf{-1.0}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+3.6}}} &
  \multicolumn{1}{c|}{{\color[HTML]{9A0000} \textbf{-0.8}}} &
  \multicolumn{1}{c|}{{\color[HTML]{9A0000} \textbf{-1.3}}} &
  {\color[HTML]{036400} \textbf{+1.4}} &
  {\color[HTML]{036400} \textbf{+0.6}} \\ \hline
 &
  SegFormer B2 &
  \multicolumn{1}{c|}{\textbf{98.5}} &
  \multicolumn{1}{c|}{87.2} &
  \multicolumn{1}{c|}{93.8} &
  \multicolumn{1}{c|}{66.8} &
  \multicolumn{1}{c|}{\textbf{93.5}} &
  \multicolumn{1}{c|}{\textbf{66.8}} &
  \textbf{95.8} &
  \multicolumn{1}{c|}{95.9} &
  \multicolumn{1}{c|}{83.2} &
  \multicolumn{1}{c|}{90.3} &
  \multicolumn{1}{c|}{\textbf{84.5}} &
  \multicolumn{1}{c|}{\textbf{74.3}} &
  \textbf{80.9} &
  \multicolumn{1}{c|}{\textbf{64.2}} &
  \multicolumn{1}{c|}{71.1} &
  \multicolumn{1}{c|}{\textbf{77.3}} &
  \multicolumn{1}{c|}{83.5} &
  \multicolumn{1}{c|}{\textbf{85.8}} &
  \textbf{68.9} &
  82.2 \\ \cline{2-22} 
 &
   &
  \multicolumn{1}{c|}{\textbf{98.5}} &
  \multicolumn{1}{c|}{\textbf{87.4}} &
  \multicolumn{1}{c|}{\textbf{93.8}} &
  \multicolumn{1}{c|}{\textbf{68.5}} &
  \multicolumn{1}{c|}{93.3} &
  \multicolumn{1}{c|}{66.3} &
  95.4 &
  \multicolumn{1}{c|}{\textbf{96.0}} &
  \multicolumn{1}{c|}{\textbf{87.0}} &
  \multicolumn{1}{c|}{\textbf{91.6}} &
  \multicolumn{1}{c|}{83.5} &
  \multicolumn{1}{c|}{73.3} &
  80.7 &
  \multicolumn{1}{c|}{64.0} &
  \multicolumn{1}{c|}{\textbf{71.7}} &
  \multicolumn{1}{c|}{76.9} &
  \multicolumn{1}{c|}{\textbf{83.7}} &
  \multicolumn{1}{c|}{85.5} &
  68.6 &
  \textbf{82.4} \\
\multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}mIOU \\ (SS)\end{tabular}}} &
  \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}SegFormer B1 \\ + \methodthree{}\end{tabular}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+0.0}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+0.2}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+0.0}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+1.7}}} &
  \multicolumn{1}{c|}{{\color[HTML]{9A0000} \textbf{-0.2}}} &
  \multicolumn{1}{c|}{{\color[HTML]{9A0000} \textbf{-0.5}}} &
  {\color[HTML]{9A0000} \textbf{-0.4}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+0.1}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+3.8}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+1.3}}} &
  \multicolumn{1}{c|}{{\color[HTML]{9A0000} \textbf{-1.0}}} &
  \multicolumn{1}{c|}{{\color[HTML]{9A0000} \textbf{-1.8}}} &
  {\color[HTML]{9A0000} \textbf{-0.2}} &
  \multicolumn{1}{c|}{{\color[HTML]{9A0000} \textbf{-0.2}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+0.6}}} &
  \multicolumn{1}{c|}{{\color[HTML]{9A0000} \textbf{-0.4}}} &
  \multicolumn{1}{c|}{{\color[HTML]{036400} \textbf{+0.2}}} &
  \multicolumn{1}{c|}{{\color[HTML]{9A0000} \textbf{-0.3}}} &
  {\color[HTML]{9A0000} \textbf{-0.3}} &
  {\color[HTML]{036400} \textbf{+0.2}} \\ \hline
\end{tabular}
\end{adjustbox}
\end{center}
\end{table}

==> main_sup.tex <==
% updated April 2002 by Antje Endemann
% Based on CVPR 07 and LNCS, with modifications by DAF, AZ and elle, 2008 and AA, 2010, and CC, 2011; TT, 2014; AAS, 2016; AAS, 2020; TH, 2022

% \documentclass[runningheads]{llncs}
% \usepackage{graphicx}
% % DO NOT USE \usepackage{times}, it will be removed by typesetters
% %\usepackage{times}

% \usepackage{tikz}
% \usepackage{comment}
% \usepackage{adjustbox}
% \usepackage{amsmath,amssymb} % define this before the line numbering.
% \usepackage{color}
% \usepackage{multirow}
% \usepackage{subcaption}
% \usepackage{pifont}
% \newcommand{\cmark}{\ding{51}}%
% \newcommand{\xmark}{\ding{55}}%
% % \usepackage[table,xcdraw]{xcolor}

% % The "axessiblity" package can be found at: https://ctan.org/pkg/axessibility?lang=en
% \usepackage[accsupp]{axessibility}  % Improves PDF readability for those with disabilities.
% % \newcommand{\ourmodel}{\textsc{OURMODE}}
% % \newcommand{\fixedgrid}{\textsc{FixedGrid}}
% % \newcommand{\JG}[1]{{\color{orange}{[Jun: #1]}}}
% % \newcommand{\SF}[1]{{\color{magenta}{[Sanja: #1]}}}
% % \newcommand{\ZW}[1]{{\color{cyan}{[Zian: #1]}}}

% % INITIAL SUBMISSION - The following two lines are NOT commented
% % CAMERA READY - Comment OUT the following two lines
% % \usepackage{ruler}
% % \usepackage[width=122mm,left=12mm,paperwidth=146mm,height=193mm,top=12mm,paperheight=217mm]{geometry}

% \usepackage{listings}
% \usepackage{xcolor}

% \definecolor{codegreen}{rgb}{0,0.6,0}
% \definecolor{codegray}{rgb}{0.5,0.5,0.5}
% \definecolor{codepurple}{rgb}{0.58,0,0.82}
% \definecolor{backcolour}{rgb}{0.95,0.95,0.92}

% \lstdefinestyle{mystyle}{
%     backgroundcolor=\color{backcolour},   
%     commentstyle=\color{codegreen},
%     keywordstyle=\color{magenta},
%     numberstyle=\tiny\color{codegray},
%     stringstyle=\color{codepurple},
%     basicstyle=\ttfamily\footnotesize,
%     breakatwhitespace=false,         
%     breaklines=true,                 
%     captionpos=b,                    
%     keepspaces=true,                 
%     numbers=left,                    
%     numbersep=5pt,                  
%     showspaces=false,                
%     showstringspaces=false,
%     showtabs=false,                  
%     tabsize=2
% }

% \lstset{style=mystyle}

% \begin{document}
% % \renewcommand\thelinenumber{\color[rgb]{0.2,0.5,0.8}\normalfont\sffamily\scriptsize\arabic{linenumber}\color[rgb]{0,0,0}}
% % \renewcommand\makeLineNumber {\hss\thelinenumber\ \hspace{6mm} \rlap{\hskip\textwidth\ \hspace{6.5mm}\thelinenumber}}
% % \linenumbers
% \pagestyle{headings}
% \mainmatter
% % \def\ECCVSubNumber{7149}  % Insert your submission number here

% \title{Improving Semantic Segmentation in Transformers using Hierarchical Inter-Level Attention} % Replace with your title\
% \subtitle{Supplementary Material}

% % INITIAL SUBMISSION 
% %\begin{comment}
% % \titlerunning{ECCV-22 submission ID \ECCVSubNumber} 
% % \authorrunning{ECCV-22 submission ID \ECCVSubNumber} 
% % \author{Anonymous ECCV submission}
% % \institute{Paper ID \ECCVSubNumber}
% %\end{comment}
% %******************

% % CAMERA READY SUBMISSION
% \titlerunning{Hierarchical Inter-Level Attention}
% \author{%
% Gary Leung $^{1,3}$  \and Jun Gao$^{1,2,3}$   \and Xiaohui Zeng $^{1,3}$  \and  Sanja Fidler$^{1,2,3}$ \vspace{8pt}\\
% \small{University of Toronto\textsuperscript{1} \quad Nvidia\textsuperscript{2} \quad Vector Institute\textsuperscript{3} } \vspace{3pt}\\
% \texttt{\scriptsize \{garyleung,jungao,xiaohui,fidler\}@cs.toronto.edu}
% }
% \authorrunning{Leung et al.}
% \institute{}
% %******************

% \newcommand{\methodfull}{{\color{purple}Hierarchical Inter-Level Attention}}
% \newcommand{\method}{{\color{purple}HILA}}
% \newcommand{\methodone}[1]{{\color{purple}HILA S(3)}}
% \newcommand{\methodthree}[1]{{\color{purple}HILA S(2,3,4)}}
% \newcommand{\uncertain}[1]{{#1}}
% \newcommand{\todo}[1]{{\color{blue}TODO: #1}}

% \newcommand{\gary}[1]{{\color{blue}{[Gary: #1]}}}
% \newcommand{\JG}[1]{{\color{orange}{[Jun: #1]}}}
% \newcommand{\SF}[1]{{\color{magenta}{[Sanja: #1]}}}
% \newcommand{\xh}[1]{{\color{teal}{[xiaohui: #1]}}}
% \maketitle
% In the supplementary material, we provide more details about our model \method{} in Section~\ref{sec:model_details}, and experimental settings in Section~\ref{sec:exp_details}. Further ablation studies are provided in Section~\ref{sec:more_ablations}, with more qualitative examples on both Cityscapes and ADE20K datasets in Section~\ref{sec:more_seg_results}.
% \input{sections/appendixA}
% \input{sections/appendixC}
% \input{sections/appendixB}
% \clearpage
% \input{sections/appendixD}
% % \input{sections/appendixE}


% \clearpage
% % ---- Bibliography ----
% %
% % BibTeX users should specify bibliography style 'splncs04'.
% % References will then be sorted and formatted in the correct style.
% %
% \bibliographystyle{splncs04}
% \bibliography{egbib}
% \end{document}

